Deep Equivariant Multi-Agent Control Barrier Functions

With multi-agent systems increasingly deployed autonomously at scale in complex environments, ensuring safety of the data-driven policies is critical. Control Barrier Functions have emerged as an effective tool for enforcing safety constraints, yet existing learning-based methods often lack in scalability, generalization and sampling efficiency as they overlook inherent geometric structures of the system. To address this gap, we introduce symmetries-infused distributed Control Barrier Functions, enforcing the satisfaction of intrinsic symmetries on learnable graph-based safety certificates. We theoretically motivate the need for equivariant parametrization of CBFs and policies, and propose a simple, yet efficient and adaptable methodology for constructing such equivariant group-modular networks via the compatible group actions. This approach encodes safety constraints in a distributed data-efficient manner, enabling zero-shot generalization to larger and denser swarms. Through extensive simulations on multi-robot navigation tasks, we demonstrate that our method outperforms state-of-the-art baselines in terms of safety, scalability, and task success rates, highlighting the importance of embedding symmetries in safe distributed neural policies.

==> files/experiments_full.tex <==
\section{Experiments}\label{sec:experiments}
% \newcolumntype{g}{>{\columncolor{Gray}}c}
\begin{table*}[t!]
  \centerfloat
\begin{adjustbox}{width=1.18\textwidth}
\begin{tabular}{c}
     \textsc{Swarm size (Agent Density $N/l^3$)}\\

\begin{tabular}{c|ccccc|ccccc|ccccc|} 
    \cline{2-16}
    & & & \textbf{8 (0.125)} & & & & & \textbf{0.25} & & & & & \textbf{64 (1)} & &   \\
    \cline{2-16}
        & Safe (\%)$\uparrow$ & Reach (\%)$\uparrow$ & Succ (\%)$\uparrow$ & Cost $\downarrow$& Rew $\uparrow$ & Safe (\%)$\uparrow$ & Reach (\%)$\uparrow$ & Succ (\%)$\uparrow$ & Cost $\downarrow$& Rew $\uparrow$ & Safe (\%)$\uparrow$ & Reach (\%)$\uparrow$ & Succ (\%)$\uparrow$ & Cost $\downarrow$& Rew $\uparrow$\\
    \hline\hline
    GCBF   & \textbf{100} & \textbf{100} & \textbf{100}& \textbf{0} (0/0) & -315.1
           & 97.5 & \textbf{100} & 97.5& 0.33 (0/2) & -311.4
           & 87.7& 99.8& 87.5& 1.09 (0.31/1.96) & -315\\
    GCBF+  & \textbf{100} & \textbf{100} & \textbf{100} & \textbf{0} (0/0) & -17.1
           & \textbf{100} & \textbf{100} & \textbf{100} & \textbf{0} (0/0) & -17.5
           & 96.5 & \textbf{100} & 96.5 & 0.23 (0/1) & -49.1\\
    dCBF &  \textbf{100}  & \textbf{100} & \textbf{100} & \textbf{0} (0/0) & -96.3
          &   \textbf{100}  & 98.125 & 98.13 & \textbf{0} (0/0) & -182.8
            &  -  & - & - & - & -\\
    cCBF &  \textbf{100}  & \textbf{100} & \textbf{100} & \textbf{0} (0/0) & -60.8
                  &   \textbf{100}  & \textbf{100} & \textbf{100} & 0 (0/0) & -120.5
                   &  -  & - & - & -  & -\\
    EGCBF(Ours)   & \textbf{100} & 91.2 & 91.2 & \textbf{0} (0/0) & -349.9
                  & \textbf{100} & 93.7 & 93.7 & \textbf{0} (0/0) & -338.5
                  & 88.4 & 94.2 & 83.4 &  1.256 (0.25/2) & -335.8\\
    EGCBF+(Ours)  & \textbf{100} & \textbf{100} &\textbf{100}& \textbf{0} (0/0) &\textbf{-9.3}
                  & \textbf{100} & \textbf{100} & \textbf{100} &  \textbf{0} (0/0) &\textbf{-14.1}
                  & \textbf{98.8} & 99.7 & \textbf{98.5}& \textbf{0.04} (0/0.21) &\textbf{-34.7}\\
    \hline

    \cline{2-16}
    & & & \textbf{128 (2)} & & & & & \textbf{256 (4)} & & & & & \textbf{512 (8)} & &   \\
    \cline{2-16}
        & Safe (\%)$\uparrow$ & Reach (\%)$\uparrow$ & Succ (\%)$\uparrow$ & Cost $\downarrow$& Rew $\uparrow$ & Safe (\%)$\uparrow$ & Reach (\%)$\uparrow$ & Succ (\%)$\uparrow$ & Cost $\downarrow$& Rew $\uparrow$ & Safe (\%)$\uparrow$ & Reach (\%)$\uparrow$ & Succ (\%)$\uparrow$ & Cost $\downarrow$& Rew $\uparrow$\\
    \hline\hline
    GCBF   & 73.9 & 99.1& 73.2& 2.47 (1.72/4.12) & -350.5
           & 52.1 & 98.5& 51.1& 5.98 (4.66/7.46) & -409.3
           & 31.6 & 96.8& 30& 11.07 (9.97/13.4) & -505.8\\
    GCBF+  & 93.6 & 99.3 & 92.9& 0.43 (0/1.31) & -104.2
           & 88.8 & \textbf{98.7} & 87.7& 0.72 (0.56/0.92) & -209.9
           & 77.8 & 96.2 & 74.5& 1.51 (1.2/1.72) & -484.2\\
    EGCBF(Ours)   & 74.1 & 96.7 & 71.7 & 2.9(2.04/3.79) & -358.1
                  & 55.1 & 97.5 & 53.6 & 5.42(4.23/7.36) & -409.8
                  & 33.1 & \textbf{98.7} & 31.7 & 10.1 (7.03/15.29)& -487.3\\
    EGCBF+(Ours)  & \textbf{97.9} &\textbf{99.5}& \textbf{97}& \textbf{0.12} (0/0.23) &  \textbf{-52.1}
                  & \textbf{94.2} & 96.6& \textbf{91.1} & \textbf{0.26} (0.06/0.51)  &\textbf{-97.8} 
                  & \textbf{89.5} & 92.1& \textbf{83.3}& \textbf{0.51} (0.23/0.73) & \textbf{-224.8} \\
    \hline    
\end{tabular}

\end{tabular}
  \end{adjustbox}
\caption{Evaluation of zero-shot transferability to growing swarm sizes and agents density for $l=4$ without obstacles. Best in class shown in bold.}
\label{table:results_scalability}
\end{table*}

We offer simulation experiments to evaluate the effect on scalability and generalization of incorporating geometric symmetries in the Graph-based CBF and policy models. 

\noindent\textbf{Environment}:
We consider a swarm of $N$ quadrotors:
\begin{align*}
    \ddot{p}_i = \mathbf{g} + \frac{1}{m}R_i \mathbf{F}_i \quad&,\quad
    \dot{\omega}_i = J^{-1}(\tau_i - \omega_i \times (J \omega_i)) \\
    \dot{R}_i =& \omega_{i,\times} R_i
\end{align*}
where $i\in I_N$ the agent tag, $m\in \mathbb{R}_{+}$ denotes the mass, $\ddot{p}_i \in \mathbb{R}^3$ is the acceleration in the world frame, $\mathbf{g}=[0,0,-9.81]^T$ is the gravitational acceleration vector, $R_i\in SO(3)$ is the rotation matrix from the body frame to the world frame, $F_i = F_3\mathbf{e}_3 \in\mathbb{R}^3,F_3\in \mathbb{R}^+$ is the thrust force in the body frame, $\omega_i \in \mathbb{R}^3$ is the angular velocity in the body frame, $J\in \mathbb{R}^{3 \times 3}$ is the inertia tensor, $\tau_i\in \mathbb{R}^3$ is the torque in the body frame for some function $\kappa$ that computes the torques induced in the local frame by the motor speeds, and $\omega_{i,\times} \in \mathbb{R}^{3 \times 3}$ is a skew-symmetric matrix associated with the angular acceleration rotated to the world frame. 
% The multi-quadrotor environment implementation is based on \cite{zhang2025gcbf+}. 
The dynamics can be compactly written in a control affine system as $\dot{x}_i(t) = f_0(x_i(t))+ f_1(x_i(t))u_i(t))$, where the state comprises of pose $\rho_i=(p_i,R_i)$ and twist $\xi_i=(\dot{p}_i,\omega_i)$, i.e. $x_i(t) = [\rho_i(t),\xi_i(t)] \in SE(3) \times \mathbb{R}^6$ and $u_i(t) = [\tau_i, F_3]\in \mathbb{R}^3 \times \mathbb{R}$.  As gravity is $O(3)$-invariant, the $SE(3)$-symmetry is broken, but the system is equivariant with respect to the subgroup of $SE(3)$
\begin{align}
    \bar{G} = \Big\{\begin{pmatrix} R^z(\theta) & \lambda  \\ 0 & 1 
    \end{pmatrix} | (\lambda,\theta)\in \mathbb{R}^3 \times S^1 \Big\}
\end{align}
which is a a Lie group, isomorphic to $SE(2) \times \mathbb{R}$, acting on $SE(3) \times \mathbb{R}^6$ via $\phi_g(x)=(g\rho,\xi)$ and on $\mathbb{R}^3 \times \mathbb{R}$ via $\psi_g(u)=(g \tau, F_3)$. If the neighborhood $\mathcal{N}_i$ is constructed via a Euclidean relative distance, for the $\bar{G}$ group induced actions Assumption \ref{assumption:G-invarinat neighborhood} stands. 

\noindent\textbf{Data collection}: In all episodes initial, target and obstacle positions are uniformly sampled over $[0,l]^3$. The training dataset $\mathcal{D}=\{D_{\text{safe},i},D_{\text{unsafe},i}\}$ is collected over numerous random configurations via an on-policy strategy that periodically executes the learned policy $\pi_{\theta}(\hat{G}_t)$ that limits distributional shift between training and inference data. Labelling the data via the distance-based safety specification may lead to infeasibility issues and computing the infinite horizon control invariant set is computationally intractable. Thus, to partition the dataset, we employ the finite reachibility approximation of \cite{zhang2025gcbf+}. If $\hat{\mathcal{{G}}}^i_t$ entails collisions, it is added in $D_{\text{unsafe},i}$. If not, $\pi_{\theta}(\hat{G}_t)$ is used to unroll sampled trajectories for a fixed horizon $T$ and, if no future collision is detected, the state is added in $D_{\text{safe},i}$, otherwise it remains unlabeled. Setting $T\rightarrow \infty$, this process would recover the infinite horizon control invariant set. The construction of graph representation of the state of the system $\hat{\mathcal{G}}_t$ is described in Section \ref{intro:graph_representation}. Notice that the torsor $\mathfrak{B}_{\bar{G}}$ of the group $\bar{G}$ is a submanifold of the state, thus, allowing for a group representation element to form from the pose to construct the $\bar{G}$-augmented graph representation $\hat{\mathcal{G}}_t$. 

\noindent\textbf{Task \& Evaluation Metrics}:
In each training episode, every quadrotor attempts to reach a designated target position of the formation while avoiding collisions with obstacles and other quadrotors. As metrics, we report the \textit{mean safety rate} (\% of agents not in collision with objects or other agents throughout the episode over all agents), \textit{mean reach rate} (\% of agents that satisfy liveness condition of reaching the target), \textit{mean success rate} (\% of agents reaching their target while remaining collision-free throughout the episode), \textit{mean cost} (average number of collisions per episode per agent) and \textit{cumulative reward} (negative sum $L_2$ loss of policy and reference controller throughout the episode). We evaluated the performance of the models in 50 episodes per swarm size and density of agents ($\approx N/l^3$). 


\subsection{Architecture \& Training}\label{section:architecture_training}
The learning framework consists of a $\bar{G}$-equivariant neural network for the policy $\pi_{\theta}(\hat{\mathcal{G}}^i_t) = \psi_{g_i} \circ m_{\theta_2}\circ \phi_{g_i^{-1}} \circ M_{\theta_1}(\hat{\mathcal{G}}^i_t)$ and a $\bar{G}$-invariant neural network for the distributed CBF $h_{\phi}(\hat{\mathcal{G}}^i_t) = m_{\phi_2}\circ \phi_{g_i^{-1}} \circ M_{\phi_1}(\hat{\mathcal{G}}^i_t)$, trained in parallel with the loss function of Section \ref{section:safe_distributed_policy}, where $M_{\theta_1},M_{\phi_1}$ are $\bar{G}$-equivariant graphormers of Section \ref{sec:equivgraphTransformer} and $m_{\theta_2},m_{\phi_2}$ standard MLPs. The structure of our networks is closely resembles \cite{zhang2025gcbf+}, with the addition of (de)canonicalizing group actions. As the torque and thrust were assumed to be in the local frame $\psi_{g_i^{-1}} \circ \pi_{\theta}(\hat{\mathcal{G}}^i_t)$. After the sampled $\hat{\mathcal{G}}^i_t$ is labeled safe/unsafe according to the aforementioned data collection scheme via $\pi_\theta$, $h_\phi,\pi_\text{nom}$ are used to solve the centralized QP-CBF of Section \ref{section:safe_distributed_policy} to produce $\pi_\text{QP}$. Finally, the errors from the loss function $\mathcal{L}$ are backpropagated to update the networks. We offer two variations of the $\bar{G}$-invariant CBF $h_\phi$: EGCBF+ and EGCBF that use $\pi_\text{QP}$ and $\pi_\text{nom}$ as reference controllers in the loss function. We use as baselines GCBF+ \cite{zhang2025gcbf+}, GCBF \cite{zhang2023gcbf} without the online policy refinement step, along with centralized and decentralized variants of CBF-QP \cite{7857061,zhang2025gcbf+}.  All models are trained with the Adam optimizer on an AMD EPYC 7313P-16 CPU @ 3000MHz and an NVIDIA A100 GPU, with $l=2$, learning rates $10^{-4}$ for the CBF and $10^{-5}$ for the policy, $\gamma=0.02$, $\eta_{\textbf{d}}=0.2$ and linear extended class-$\mathcal{K}$ function $\alpha(\cdot)=\cdot$. All other hyperparameters regarding the architecture and training algorithm follow \cite{zhang2025gcbf+}.

\begin{figure}[h!]
    \centering
    \includegraphics[trim={1cm 0.2cm 1cm 1.5cm},clip,width=1\linewidth]{scalability_plot_safety.png}
    \caption{Safety rates for zero-shot scalability evaluations for $l=4$ and 5 obstacles. The safety rates are dropping only slightly compared to the obstacle-free experiments, suggesting that obstacle avoidance is easier for the static parts of the graph than with other agents (that requires coordination). Still, the symmetry-enhanced models outperform their non-symmetric counterparts.}
    \label{fig:scalability}
\end{figure}
\subsection{Generalization \& Scalability Analysis}
We offer experiments to evaluate the scalability, generalization and efficiency of the proposed symmetries-enhanced network. The models $\pi_\theta,h_\phi$ were trained in navigation scenarios with a swarm comprising of 8 robots, $l=2$ (0.125 estimated density) and 5 obstacles for 1000 steps, and tested with zero-shot transfer on swarms of 8-512 robots, with $l=4$ (estimated density ranging from 0.125 to 8, an increase of 6400\%), in environments without obstacles (summarized in Table \ref{table:results_scalability}) and with 8 obstacles (see Figure \ref{fig:scalability}). We were unable to test cCBF-QP and dCBF-QP for more than 16 robots as solving the QP exceeded computation time and memory restrictions (the dCBF-QP would theoretically run on multiple robots separately, and thus would run for more robots, but our simulation is run centralized on one node). For 8 robots, same as during training, all methods guarantee safety, though the hand-crafted cCBF-QP, dCBF-QP, and EGCBF, GCBF (trained with the nominal controller instead of the QP solution) are overly conservative, as indicated by the high reach rate but low reward. As $N$ increases, EGCBF and GCBF safety and success rates drop significantly (by $\approx 70\%$ and 60\% respectively), while the reach rate remains high (the low rewards suggest a slow target reaching with possible deadlocks). This can be explained by the fact that the nominal controller is computed without any notion of safety, thus the control and safety terms in the loss function are inconsistent. Figure \ref{fig:scalability} demonstrates the significance of the training the models with reference controllers that account for safety. The safety rates of (E)GCBF drop exponentially, contrary to (E)GCBF+ that is almost linear. However, as environments get more cluttered, (E)GCBF+ reach rates drop faster, as $\pi_\text{nom}$ that ensures liveness is unable to resolve deadlocks when adapted by the $\pi_{QP}$.   
Overall, the symmetry-enhanced EGCBF+ outperforms the baselines across all sizes-densities, attaining higher rewards and exhibiting to fewer collisions (for 512 drones the EGCBF+ collision rate drops to $\approx 90\%$ compared to $<78\%$ for the baselines) than the baselines and increased success rate, as the embedded symmetries that are leveraged locally are not affected by the size of the swarm. It is indicative that, for 512 drones, EGCBF+ leads to $0.5$ collisions per drone while the non-equivariant more than $1.5$.
\begin{figure}[h!]
    \centering
    \includegraphics[trim={2.4cm 2cm 2cm 3cm},clip,width=\linewidth]{W&B Chart 3_1_2025, 11_31_39 AM.png}
    \caption{$G$-equivariant policies converge faster than the non-equivariant ones.}
    \label{convergence}
\end{figure}
The equivariant policies exploit the structure of the collision avoidance and liveness specification to shrink the hypothesis class and, thus, effectively restricting the models and leading to sampling efficient and accurate learning of collision avoidance
without loss of expressivity of the final policy. EGCBF(+) converge faster (Figure \ref{convergence} depicts reach rate during training) than GCBF(+) as the $G$-equivalent state-action pairs appear.





